Advancements on SEFE and Partitioned Book Embedding Problems

In this work we investigate the complexity of some problems related to the {\em Simultaneous Embedding with Fixed Edges} (SEFE) of $k$ planar graphs and the PARTITIONED $k$-PAGE BOOK EMBEDDING (PBE-$k$) problems, which are known to be equivalent under certain conditions. While the computational complexity of SEFE for $k=2$ is still a central open question in Graph Drawing, the problem is NP-complete for $k \geq 3$ [Gassner {\em et al.}, WG '06], even if the intersection graph is the same for each pair of graphs ({\em sunflower intersection}) [Schaefer, JGAA (2013)]. We improve on these results by proving that SEFE with $k \geq 3$ and sunflower intersection is NP-complete even when the intersection graph is a tree and all the input graphs are biconnected. Also, we prove NP-completeness for $k \geq 3$ of problem PBE-$k$ and of problem PARTITIONED T-COHERENT $k$-PAGE BOOK EMBEDDING (PTBE-$k$) - that is the generalization of PBE-$k$ in which the ordering of the vertices on the spine is constrained by a tree $T$ - even when two input graphs are biconnected. Further, we provide a linear-time algorithm for PTBE-$k$ when $k-1$ pages are assigned a connected graph. Finally, we prove that the problem of maximizing the number of edges that are drawn the same in a SEFE of two graphs is NP-complete in several restricted settings ({\em optimization version of SEFE}, Open Problem $9$, Chapter $11$ of the Handbook of Graph Drawing and Visualization).

==> makefile <==
finalname = main

psfiles = \


pdf:
	pdflatex $(finalname).tex



startup:
	xemacs $(finalname).tex &
	xdvi $(finalname) &
	xfig -bg white -fg black &

clean:
	rm -f $(psfiles)
	rm -f $(finalname).ps
	rm -f tmp-data/*.avg
	rm -f tmp-data/*.txt
	rm -f src-data/*.tmp
	rm -f *~
	rm -f *.bak
	rm -f figures/*.bak
	rm -f *.toc
	rm -f *.aux
	rm -f *.blg
	rm -f *.dvi
	rm -f *.log
	rm -f *.out
	rm -f *.backup
	rm -f *.pdf

bib: 
	pdflatex $(finalname).tex
	bibtex $(finalname)
	pdflatex $(finalname).tex
	pdflatex $(finalname).tex

ps: $(finalname)
	dvips -t a4 $(finalname).dvi -o # -pp 6 -t a4

#	dvips -t letter $(finalname).dvi -o



print: ps
	lpr -Ppolaris -h $(finalname).ps

